Exploiting Intrinsic Kinematic Null Space for Supernumerary Robotic Limbs Control

Supernumerary robotic limbs (SRLs) gained increasing interest in the last years for their applicability as healthcare and assistive technologies. These devices can either support or augment human sensorimotor capabilities, allowing users to complete tasks that are more complex than those feasible for their natural limbs. However, for a successful coordination between natural and artificial limbs, intuitiveness of interaction and perception of autonomy are key enabling features, especially for people suffering from motor disorders and impairments. The development of suitable human-robot interfaces is thus fundamental to foster the adoption of SRLs. With this work, we describe how to control an extra degree of freedom by taking advantage of what we defined the Intrinsic Kinematic Null Space, i.e. the redundancy of the human kinematic chain involved in the ongoing task. Obtained results demonstrated that the proposed control strategy is effective for performing complex tasks with a supernumerary robotic finger, and that practice improves users' control ability.

==> img/radiiProfile.tex <==

\begin{figure}[b!]
\centering\
\null \hfill
\subfloat[]{\label{fig:Exp1Profile}\includegraphics[width=0.48\columnwidth]{img/radiiProfile.eps}}
\hfill \null 
\null \hfill
\subfloat[]{\label{FIG:Exp1Error}\includegraphics[width=0.48\columnwidth]{img/radiiError.eps}}
\hfill \null
\caption{Experiment 2 (parallel tasks case). (a) Desired and actual radius value in a representative trial, reported in blue and red, respectively. (b) The  error in accomplishing the primary task, \iec the distance between the two spheres centres. \label{FIG:expSfera}}
\end{figure}
